The Fermi-LAT Light Curve Repository: A resource for the time-domain and multi-messenger communities

For over 15 years the Fermi Large Area Telescope (Fermi-LAT) has been monitoring the entire high-energy gamma-ray sky, providing the best sampled 0.1 -- $>1$ TeV photons to this day. As a result, the Fermi-LAT has been serving the time-domain and multi-messenger community as the main source of gamma-ray activity alerts. All of this makes the Fermi-LAT a key instrument towards understanding the underlying physics behind the most extreme objects in the universe. However, generating mission-long LAT light curves can be very computationally expensive. The Fermi-LAT light curve repository (LCR) tackles this issue. The LCR is a public library of gamma-ray light curves for 1525 Fermi-LAT sources deemed variable in the 4FGL-DR2 catalog. The repository consists of light curves on timescales of days, weeks, and months, generated through a full-likelihood unbinned analysis of the source and surrounding region, providing flux and photon index measurements for each time interval. Hosted at NASA's FSSC, the library provides users with access to this continually updated light curve data, further serving as a resource to the time-domain and multi-messenger communities.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

